Boosted Density Estimation Remastered

There has recently been a steady increase in the number iterative approaches to density estimation. However, an accompanying burst of formal convergence guarantees has not followed; all results pay the price of heavy assumptions which are often unrealistic or hard to check. The Generative Adversarial Network (GAN) literature --- seemingly orthogonal to the aforementioned pursuit --- has had the side effect of a renewed interest in variational divergence minimisation (notably $f$-GAN). We show that by introducing a weak learning assumption (in the sense of the classical boosting framework) we are able to import some recent results from the GAN literature to develop an iterative boosted density estimation algorithm, including formal convergence results with rates, that does not suffer the shortcomings other approaches. We show that the density fit is an exponential family, and as part of our analysis obtain an improved variational characterisation of $f$-GAN.

==> content/experiments.tex <==
\section{Experiments}\label{sec:experiments}
\begin{figure}[p]
    \centering
    \subfloat[Gaussian ring]{
        \begin{tabular}{cc}
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5]
            \addplot graphics [xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-ring_00-Plots_contour-xlim_-6_5_to_6_5-ylim_-6_5_to_6_5};
            \node[anchor=south west] at (current axis.south west) {$t=0$};
        \end{axis}\end{tikzpicture}
        &
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5]
            \addplot graphics [xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-ring_01-Plots_contour-xlim_-6_5_to_6_5-ylim_-6_5_to_6_5};
            \node[anchor=south west] at (current axis.south west) {$t=1$};
        \end{axis}\end{tikzpicture}\\
        %
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5]
            \addplot graphics [xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-ring_02-Plots_contour-xlim_-6_5_to_6_5-ylim_-6_5_to_6_5};
            \node[anchor=south west] at (current axis.south west) {$t=2$};
        \end{axis}\end{tikzpicture}
        &
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5]
            \addplot graphics [xmin=-6.5, xmax=6.5, ymin=-6.5, ymax=6.5, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-ring_03-Plots_contour-xlim_-6_5_to_6_5-ylim_-6_5_to_6_5};
            \node[anchor=south west] at (current axis.south west) {$t=3$};
        \end{axis}\end{tikzpicture}
    \end{tabular}
    }
    \subfloat[Randomly placed Gaussians]{
        \begin{tabular}{cc}
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-10, xmax=10, ymin=-10, ymax=10]
            \addplot graphics [xmin=-10, xmax=10, ymin=-10, ymax=10, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-rand_00-Plots_contour-xlim_-10_0_to_10_0-ylim_-10_0_to_10_0};
            \node[anchor=south west] at (current axis.south west) {$t=0$};
        \end{axis}\end{tikzpicture}
        &
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-10, xmax=10, ymin=-10, ymax=10]
            \addplot graphics [xmin=-10, xmax=10, ymin=-10, ymax=10, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-rand_01-Plots_contour-xlim_-10_0_to_10_0-ylim_-10_0_to_10_0};
            \node[anchor=south west] at (current axis.south west) {$t=1$};
        \end{axis}\end{tikzpicture}\\
        %
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-10, xmax=10, ymin=-10, ymax=10]
            \addplot graphics [xmin=-10, xmax=10, ymin=-10, ymax=10, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-rand_02-Plots_contour-xlim_-10_0_to_10_0-ylim_-10_0_to_10_0};
            \node[anchor=south west] at (current axis.south west) {$t=2$};
        \end{axis}\end{tikzpicture}
        &
        \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-10, xmax=10, ymin=-10, ymax=10]
            \addplot graphics [xmin=-10, xmax=10, ymin=-10, ymax=10, includegraphics={trim=16 16 20 16, clip}] 
            {plots/visualising_convergence/visualising_convergence-rand_05-Plots_contour-xlim_-10_0_to_10_0-ylim_-10_0_to_10_0};
            \node[anchor=south west] at (current axis.south west) {$t=3$};
        \end{axis}\end{tikzpicture}
    \end{tabular}
    }
    \caption{Visualising the convergence of $Q_t$ to $P$.}\label{fig:vis_cvg}    
\end{figure}
Our experiments take palce $\cal X \defas \R^2$. We use the following simple neural network classifier
\begin{gather}
    D_t:\cal X \xrightarrow[\textrm{dense}]{\tanh} \R^{10}\xrightarrow[\textrm{dense}]{\tanh} \R\xrightarrow{\sigma} (0,1),\label{eq:simplenn}
\end{gather}
which we transform into a density ratio, $d_t$, by substituting the sigmoid activation with an exponential function (cf.\ \autoref{sec:preliminaries}).  To generate samples from $Q_{t-1}$ for training we use random walk Metropolis--Hastings. The network $D_t$ is trained with 10k samples each from $P$ and $Q_{t-1}$ using Nesterov's accelerated gradient descent $\eta = 0.01$ for 600 epochs with cross-entropy loss. One quarter of the pooled $P$ and $Q_{t-1}$ samples are reserved for a test set, which we use for early stopping.

\subsection{Metrics}

% \paragraph{Metrics} 
To compare our results with \citet{tgbssAB} we compute their coverage
metric\footnote{This is easier in our setting since we have direct
  access to the density $\d Q$, where \citet{tgbssAB} estimate it with
  a cross-validated kernel density estimator.}: $C_{\kappa}(P,Q)
  \defas P\rbr{\lev_{>\beta}\d Q}$, where  $Q\rbr{\lev_{>\beta}\d Q} = \kappa,$
and $\kappa\in[0,1]$. That is, we first find a set where most of the mass of $Q$ lies, $\lev_{>\beta}\d Q$, then look at how much of the mass of $P$ resides there. In addition to $C_{\kappa}$ we also compute the negative log-likelihod (NLL) $\E_{P}[-\log \d Q]$ and KL divergence.

\subsection{Convergence}

At each iteration $t$ we train a new binary classifier $c_t$; we use this classifier to push $Q_{t-1}$ towards $P$. As $Q_t$ gets closer to $P$ it becomes harder and harder to build a good classifier to tell them apart. This is easy to see in \autoref{fig:cvg}. As the KL divergence decrease with $t$, \autoref{fig:cvg_c}, the minimal cross entropy we're able to achieve over the course of training increases \autoref{fig:cvg_q}. 

Dually we can interpret convergence in terms of the difficulty of constructing the weak lerner from \autoref{sec:boosted_density_estimation}. In \autoref{fig:cvg_c} we plot the quantites $\mup$ and $\muq t$. At the beginning of each iteration of training either $\mup$ or $\muq t$ is negative, indicating that the classifier we're learning does not yet satisfy \ref{wla}, by the end of training both are positive. Furthermore, as with training iterations $t$ the maximal value we're able to achieve in $\min\cbr{\mup, \muq t}$ decreases, meaning that we are learning weaker and weaker classifiers, until when we have converged, the benefit from additional training iterations is negligable. We plot the density for several iterations of boosting in \autoref{fig:vis_cvg}.
\begin{figure}
    \begin{center}
        \subfloat[%Convergence metrics:  
        \ref{pgf:kl} $\kl(P,Q_t)$; \ref{pgf:coverage} $C_{95\%}(P,Q_t)$; \ref{pgf:negative_log_likelihood} NLL.]{\label{fig:cvg_q}
            \begin{tikzpicture}\begin{axis}[julia_convergence_plot, xmin=0.0, xmax=10, ymin=0, ymax=6, extra y ticks={1}]
                % trim=left bottom right top 
                \addplot[forget plot] graphics [xmin=0, xmax=10, ymin=0, ymax=6, includegraphics={trim=16 16 20 16, clip}] {plots/convergence_analysis/convergence_analysis-coverage_metrics_ring-RecipesBase_plot-xlim_0_to_10-ylim_0_to_6};
                \addlegendimage{no markers, Red}
                \label{pgf:kl}
                \addlegendimage{no markers, Blue}
                \label{pgf:coverage}
                \addlegendimage{no markers, Green}
                \label{pgf:negative_log_likelihood}
            \end{axis}\end{tikzpicture}}
        \quad
        \subfloat[%Classifier metrics: 
        \ref{pgf:cross_entropy} cross entropy; \ref{pgf:mu_p} $\mup$;  \ref{pgf:mu_q} $\muq t$.]{\label{fig:cvg_c}
            \begin{tikzpicture}\begin{axis}[julia_convergence_plot, xmin=0, xmax=8, ymin=-0.5, ymax=1.6,]
                \addplot[forget plot] graphics [xmin=0, xmax=10, ymin=-0.3, ymax=1.6, includegraphics={trim=16 16 20 16, clip}] {plots/convergence_analysis/convergence_analysis-train_metrics_ring-RecipesBase_plot-xlim_0_to_10-ylim_-0_3_to_1_6};
                % \addlegendimage{no markers, red}
                % \legend{cross entropy, $\mup$, $\muq t$}
                \addlegendimage{no markers, Red}
                \label{pgf:cross_entropy}
                \addlegendimage{no markers, Green}
                \label{pgf:mu_p}
                \addlegendimage{no markers, Blue}
                \label{pgf:mu_q}
            \end{axis}\end{tikzpicture}
            }
    \end{center}
    \caption{Metrics for analysing convergence over several iterations of boosting. In \protect\subref{fig:cvg_q} we show the coverage metrics at each iteration $t$. In \protect\subref{fig:cvg_c} we plot the  metrics to evaluating the classifier on at batch while training the neural network, between boosting iterations $t$.}
    \label{fig:cvg}
\end{figure}



\subsection{The Effect of the Activation Function}
The target distribution $P$ is a mixture of eight isotropic Gaussians arranged in a ring in $\cal X \defas \R^2$. We modity our simple neural classifier \eqref{eq:simplenn} by varying the activations on the two hidden layers of \eqref{eq:simplenn}. We compare the resulting densitites at $t=5$ for a selection of activation functions $a$. Contour plots are provided in \autoref{fig:activation} for ReLU, Tanh, and Softplus. We also tried but have not plotted: ELU with $a=1$, this looked very similar to Softplus; Leaky ReLU, very similar to ordinary ReLU; and Sigmoid, which was disastrous, converging to a single mode distribution somewhat like a Gaussian. 
\begin{figure}
    \begin{center}
        \subfloat[Target]{\label{fig:activation_target}
            \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6]
                % trim=left bottom right top 
                \addplot graphics [xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6, includegraphics={trim=16 16 20 16, clip}] 
                {plots/activation_comparison/activation_comparison-control-Plots_contour-lims_-6_5_to_6_6};
            \end{axis}\end{tikzpicture}}
        \subfloat[ReLU]{\label{fig:activation_relu}
            \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6]
                % trim=left bottom right top 
                \addplot graphics [xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6, includegraphics={trim=16 16 20 16, clip}] 
                {plots/activation_comparison/activation_comparison-NNlib_relu-Plots_contour-lims_-6_5_to_6_6};
            \end{axis}\end{tikzpicture}}
        \subfloat[Tanh]{\label{fig:activation_tanh}
            \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6]
                % trim=left bottom right top 
                \addplot graphics [xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6, includegraphics={trim=16 16 20 16, clip}] 
                {plots/activation_comparison/activation_comparison-tanh-Plots_contour-lims_-6_5_to_6_6};
            \end{axis}\end{tikzpicture}}
        \subfloat[Softplus]{\label{fig:activation_softplus}
            \begin{tikzpicture}\begin{axis}[julia_contour_plot, xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6]
                % trim=left bottom right top 
                \addplot graphics [xmin=-6.5, xmax=6.6, ymin=-6.5, ymax=6.6, includegraphics={trim=16 16 20 16, clip}] 
                {plots/activation_comparison/activation_comparison-NNlib_softplus-Plots_contour-lims_-6_5_to_6_6};
            \end{axis}\end{tikzpicture}}
    \end{center}
    \caption{The effect of different activation functions.}
    \label{fig:activation}
\end{figure}

\subsection{Comparison with \protect{\citet{tgbssAB}}} 
To compare the performance with \textsc{AdaGAN} we use the exact same network configuration as \citet[\S4.1]{tgbssAB} for the discriminator and generator. That is
\begin{align}
    & G_t^{\textrm{AdG}}:\cal L \xrightarrow[\textrm{dense}]{\textrm{ReLU}} \R^{10}\xrightarrow[\textrm{dense}]{\textrm{ReLU}}\R^{5} \to \cal X,\\
    & D_t^{\textrm{AdG}}:\cal X \xrightarrow[\textrm{dense}]{\textrm{ReLU}} \R^{20}\xrightarrow[\textrm{dense}]{\textrm{ReLU}}\R^{10}\xrightarrow[\textrm{dense}]{\textrm{ReLU}} \R\xrightarrow{\sigma} (0,1),\label{eq:adag_disc}
\end{align}  
where $\cal L = \R^5$. At the beginning of each experimental run, the target distribution $P$ is a mixture of 10 randomly located isotropic Gaussians with variance of $1/2$. The procedure is as follows: We sample 10k examples from $P$, these same examples are then used to run \textsc{AdaGAN} and OURTHING each for 10 iterations. Since we are training on only 10k examples, compared to their 64k examples  \citep[\S4.1.1]{tgbssAB}, we run their training routine for an extra six epochs with early stopping. 

Negative Log-Likelihood and $C_{95\%}$ are plotted in \autoref{fig:adagan_comparison}. Early on \adabodeEST\ easily outperforms \textsc{AdaGAN}, which gradually only catches up at iteration 10. However our architecture \eqref{eq:simplenn} posesses less than a fifth of the parameters of \textsc{AdaGAN}. For this reason we reran the experiment using \eqref{eq:adag_disc} for the \adabodeEST\ classifier with a fixed $\alpha_t = 0.7$. The results are shown in \autoref{fig:adagan_comparison2} wherein we achieve dramatically better performance both in NLL and $C_{95\%}$.
\begin{figure}
    \begin{center}
        \subfloat[NLL (lower is better)]{\label{fig:adagan_comparison_nll}
            \begin{tikzpicture}\begin{axis}[julia_convergence_plot, xmin=1.0, xmax=10.0, ymin=3.0, ymax=10.0]
                \addplot graphics [xmin=0.0, xmax=10.0, ymin=3.0, ymax=10.0, includegraphics={trim=16 16 20 16, clip}] 
                {plots/adagan_comparison/adagan_comparison-likelihood-RecipesBase_plot-xlim_0_to_10-ylim_3_to_10};
                \addlegendimage{no markers, Red}
                \label{pgf:adagan}
                \addlegendimage{no markers, Cyan}
                \label{pgf:our_thing}
            \end{axis}\end{tikzpicture}}
        \quad
        \subfloat[Coverage $C_{95\%}$ (higher is better).]{\label{fig:adagan_comparison_coverage}
            \begin{tikzpicture}\begin{axis}[julia_convergence_plot, xmin=1.0, xmax=10.0, ymin=0.0, ymax=1.0]
                \addplot graphics [xmin=0.0, xmax=10.0, ymin=0.0, ymax=1.0, includegraphics={trim=16 16 20 16, clip}] 
                {plots/adagan_comparison/adagan_comparison-coverage-RecipesBase_plot-xlim_0_to_10-ylim_0_to_1};
            \end{axis}\end{tikzpicture}}
    \end{center}
    \caption{\textsc{AdaGAN} comparison. Feint lines are individual runs of each algorith, the solid lines are the median:  \ref{pgf:adagan} \textsc{AdaGAN}; \ref{pgf:our_thing} \adabodeEST.}\label{fig:adagan_comparison}
    \begin{center}
        \subfloat[NLL (lower is better).]{\label{fig:adagan_comparison_nll2}
            \begin{tikzpicture}\begin{axis}[julia_convergence_plot, xmin=1.0, xmax=10.0, ymin=3.0, ymax=10.0]
                \addplot graphics [xmin=0.0, xmax=10.0, ymin=3.0, ymax=10.0, includegraphics={trim=16 16 20 16, clip}] 
                {plots/adagan_comparison_big/adagan_comparison_big-likelihood-RecipesBase_plot-xlim_0_to_10-ylim_3_to_10};
                \addlegendimage{no markers, Red}
                \label{pgf:adagan2}
                \addlegendimage{no markers, Cyan}
                \label{pgf:our_thing2}
            \end{axis}\end{tikzpicture}}
        \quad
        \subfloat[Coverage $C_{95\%}$ (higher is better).]{\label{fig:adagan_comparison_coverage2}
            \begin{tikzpicture}\begin{axis}[julia_convergence_plot, xmin=1.0, xmax=10.0, ymin=0.0, ymax=1.0]
                \addplot graphics [xmin=0.0, xmax=10.0, ymin=0.0, ymax=1.0, includegraphics={trim=16 16 20 16, clip}] 
                {plots/adagan_comparison_big/adagan_comparison_big-coverage-RecipesBase_plot-xlim_0_to_10-ylim_0_to_1};
            \end{axis}\end{tikzpicture}}
    \end{center}
    \caption{\textsc{AdaGAN} comparison using the AdaGAN discriminator architecture \eqref{eq:adag_disc}. Feint lines are individual runs of each algorith, the solid lines are the median.}\label{fig:adagan_comparison2}
\end{figure}

==> content/introduction.tex <==
\section{Introduction}
Learning a distribution $Q$ to approximate a \textit{true} distribution $P$ over a space $\cal X$ entails potentially two difficulties: \textit{Firstly}, ensuring formally that $Q$ is close to $P$. That is, guaranteeing
\begin{gather}
    I(P,Q)  \leq  C,\label{destBOUND}
\end{gather}
where $I$ is any suitable form of divergence, and $C$ can take a variety of forms. \textit{Secondly}, devising an easy way to generate samples from $Q$. There is no approach to date that satisfies both objectives for both $C$ sufficiently small with reasonable assumptions and a sampling scheme sufficiently efficiently in the worst cases. Recent approaches, formal and/or experimental, have promoted the idea that $Q$ can be learned in an iterative way using density iterates obtained from an \textit{oracle}, and analyzed convergence alongside the original boosting theory \citep[and references therein]{grover2017boosted,gwfbdBV,lkgrBV,mfaVB,tgbssAB}. Experimentally, successful applications have essentially be framed in the context of variational inference \citep{gwfbdBV,lkgrBV,mfaVB} or Generative Adversarial Networks (GANs) \citep{tgbssAB}. To our knowledge, there is no such black box method whose convergence has been proven towards the optimum and with realistic and/or easily checkable assumptions. For example, the strongest of the convergence results, which exhibit geometric rates, assumes that the iterates are close to the optimum sought \citep{tgbssAB}. All previous results attaining at least sublinear convergence rates --- that represent the main body of results in the field --- also make strong assumptions about the parameters and models at hand. It is therefore not just about obtaining efficient black boxes: the question as to whether substantial convergence holds under some sufficiently weak assumptions is also yet to be framed and answered.

Historically, when the statistical and computational requirements of supervised learning were still a challenge, the boosting approach to PAC learning \citep{kTO,vAT}, and its first formal proof \citep{sTS} elegantly showed that all one needs is in fact a weak learner, returning classifiers with the sole constraint to be slightly different than the unbiased coin. In a sense, any weaker than this requirement would allow just plain random guessing and would thus not be qualifiable as ``learning''. 

Our main formal contribution shows that the \textit{same} weak learners can be used to solve the density learning problem in the boosting framework --- that is, we built $Q$ using \textit{classifiers}. We attain convergence rates that compete with sublinear rates, with assumptions far weaker than those of previous results. Modulo an additional weak assumption on the distribution of errors, that we call weak dominance, we reach geometric convergence rates that compete with the best known without assuming anything about the relationship of the iterates to the optimum $P$, nor about the location of the optimum \citep{gmSC}. In the course of this contribution, we provide additional results of independent interest, including a better characterization of the variational $f$-GANs objective of \citet{nowozin2016f} and a proof that the $Q$ we learn belongs to exponential families, with a sufficient statistics defined by the classifiers' mappings. Hence,
\textit{we learn distributions whose analytical form is well studied and simple but parameterized on a statistical manifold which can be as complex as \textit{e.g.} permitted by deep learning.}

We complete our contribution with an experimental validation of our results, including the implementation of a sampler for $Q$ fit to small to moderate domains that we test on simulated problems. Our results display the ability to rapidly capture modes through iterations --- which is a key problem for generative approaches \citep{tgbssAB}. A comparison with AdaGAN displays that we converge much faster early to good solution, with architectures that represent only the fifth's of AdaGAN's size.

\vspace{\baselineskip}

% The rest of this paper is as follows. In \autoref{sec:related}, we summarize related work in the area. In \autoref{sec:preliminaries}, we provide preliminary definitions and results. In \autoref{sec:boosted_density_estimation}, we develop our theoretical results, and in \autoref{sec:experiments} we present experiments. We discuss our findings in \autoref{sec:discussion}. A final section (\autoref{sec:conclusion}) concludes the paper. This paper is self-contained but to keep it readable, all formal proofs are deferred to the appendices, starting p.~\pageref{sec:allproofs}.

==> content/related_work.tex <==
\section{Related work}\label{sec:related}

In learning a density, it is remarkable that most previous approaches \citep[and references therein]{grover2017boosted,gwfbdBV,lbMD,mfaVB,rsBD,tgbssAB,zSG} have investigated a single update rule, not unlike Frank--Wolfe optimisation:
\begin{gather}
    \cramped{\forall{\alpha_t \in [0,1]} 
    Q_{t+1} = f(\alpha_t g(c_t) + (1-\alpha_t) g(Q_t)),}
    \hphantom{(2)}
    \label{eq:genupdatebden}
\end{gather}
where $g$ is in general (but not always) the identity. \citet{grover2017boosted} is one (recent) rare exception to \eqref{eq:genupdatebden} wherein alternative choices are explored. Apart from the fact that they would rely on gradient-based optimisation in the general case, few results are accompanied by convergence proofs, and even less display convergence \textit{rates}, which are mandatory in a boosting setting \citep{gwfbdBV,lbMD,rsBD,tgbssAB,zSG}.

Two categories of convergence results results prevail: bounds of the form $I(P,Q_T) \leq \inf_Q I(P,Q) + J/T$ for $J>0$, as pioneered by \citet{lbMD}; and tighter geometric convergence bounds of the type $I(P,Q_T) \leq (1-J)^T I(P, Q_0)$ for $J \in [0,1]$ \citep[e.g.][]{tgbssAB}.  The quantity $J$ can take a variety of forms depending on the domain's parameters. Several approaches in \eqref{eq:genupdatebden} and $J$ employ parameters that are not explicitly computable: they can be the solution to alternative optimization problems \citep{gwfbdBV,neDE,rsBD,zSG} (and therefore require additional algorithmic machinery which, if not carefully designed, may break convergence guarantees \citep{mfaVB}), or they simply may not be available in closed form in general \citep[Theorems 1, 2]{tgbssAB}. 

To establish convergence and/or bound convergence by a rate, \textit{all} approaches necessarily make structural assumptions or approximations on the parameters involved in \eqref{eq:genupdatebden} or \eqref{destBOUND}. These can be on the (local) variation of $I$ \citep{gwfbdBV,neDE,zSG}; the true density $P$ or the updates $Q_t$ \citep{grover2017boosted,gwfbdBV,lbMD}; the mixing parameter $\alpha_t$ \citep{mfaVB,tgbssAB}; the weak learners $c_t$ \citep{grover2017boosted,rsBD,tgbssAB,zSG}; the previous updates, $(c_j)_{j\leq t}$ ,\citep{rsBD}; and so on. The price to get the best geometric convergence bounds is in fact heavy considering that the update $c_t$ is in all cases required to be close to the optimal one \citep[Corollaries 2, 3]{tgbssAB}. 

To our knowledge, no previous work relaxes these assumptions yet still achieves the best possible convergence rates --- which would indeed look like weak learning. It must be kept in mind, however, that for many of these works, the objective is also to get an efficient black box for sampling from $P$. With regards to this objective, boosting approaches like those of \citet{mfaVB,tgbssAB} stand out, \citet{tgbssAB} certainly being the closest to ours in their formal setting.

==> tikz_figures/activation_target.dpth_22.36.55 <==
0.0pt
\pgfexternal@restore {\def \pgfexternaltrimleft {-0.2pt}}
\pgfexternal@restore {\def \pgfexternaltrimright {-0.2pt}}


==> tikz_figures/activation_target.md5_22.36.54 <==
\def \tikzexternallastkey {888ECE799879C3B2202DF8048B7963A6}%

